Disc breaking through forced eccentricity growth

Motivated by misaligned discs observed in eccentric orbit Be/X-ray binaries, we examine the evolution of a retrograde disc around one component of an eccentric binary with hydrodynamic simulations, $n$-body simulations and linear theory. Forced eccentricity growth from the eccentric orbit binary causes the initially circular disk to undergo eccentricity oscillations. A retrograde disc becomes more radially extended, more highly eccentric and undergoes more rapid apsidal precession compared to a prograde disc. We find that a retrograde disc can be subject to disc breaking where the disc forms two rings with different eccentricities and longitude of periastrons while remaining coplanar. This could have implications for the lightcurves and the X-ray outbursts observed in Be/X-ray binaries.

==> response.tex <==
Response to reviewer report: 

We thank the reviewer for the useful comments, which we have fully addressed below. The comments have greatly improved the clarity of the letter, and we hope the letter is now to the satisfaction of the reviewer, and ready for publication. 

Introduction: 

1) first paragraph – what does “closer to retrograde” mean? Intuitively, I have a hard time sorting this phrase out. I understand the geometry and the way that retrograde is defined in terms of degrees in this work. However, I don’t quite understand how a disc can be “closer” to retrograde. Isn’t the disc either prograde or retrograde? I would really appreciate some explanation to help me understand why the authors explain disc rotation in this way.

RESPONSE: We have removed this phrase. In the first paragraph of the introduction we have modified the description of how a disc's inclination can evolve towards retrograde coplanar. 

2) I also wondered about the detail in the second paragraph in the introduction. “For a circular orbit binary, we found that the larger disc can be unstable to tilting in the outer regions (Overton et al. 2023). “ Since you are examining retrograde orbits that can grow bigger, and the fact that you study co-planar discs in this work, how might this tilting that you mention affect your results since here you ignore tilting. I was wondering why this point was made. (A second minor point about this phrase is that the wording is strange since you state, “we found” since the “we” should technically be Overton et al. 2023, I believe.)

RESPONSE: We have clarified the second paragraph of the introduction to emphasize that tilting is not prohibited, but the effects driving the tilt instability in the circular binary case may no longer work. This point is made to explain the context of this work as a continuation of previous work on retrograde disc dynamics. We have also changed the word "we" to Overton et al. 2023. 

3) The phrase “by forced eccentricity” is not clear. What is exactly is forced eccentricity. Could you please consider add a brief explanation in addition to the Martin 2020 reference. (A related minor point is in this last sentence of the paragraph, the word eccentric (or derivatives of this word) appears three times.)

RESPONSE: A brief description of forced eccentricity is added in paragraph 2 of the introduction. 

Section 2: 

4) Figure 1: This figure is not introduced and explained. Figure 2 and Figure 3 are mentioned before Figure 1, I believe.

RESPONSE: The previous figure 1 has been moved down to figure 3. We have added more description of this figure to the text.

5) Figure 1: I also had trouble trying to “see” the breaking features from the plots of the surface density. Where are the breaks? I wondered if it might be better if this plot was made with surface eccentricity instead of surface density or perhaps a 2D plot of eccentricity along with the density plot might be helpful? This way you can explain to the reader where the breaks are. I spent a long time trying to understand where breaks are. Given the breaks are tied to the fundamental results in the paper, it would be helpful to see where they are.

RESPONSE: In order to better show the break, we have changed the color map of figure 3 (previously figure 1), to better show the contrast in the low density break-region. Additionally, we have changed the axes in figure 1 (previously figure 2) so that the behavior of the retrograde disc between a semi major axis of 40 to 60 solar radii is more clear. We have also changed the plot to focus on the time during the break, by choosing to plot more lines at later times, rather than evenly spaced in the simulation. Additionally, we have slightly changed the line styles/colors to be more easily visible. We believe this plot now better shows the dip in the surface density, which is where the break occurs. 

6) Figure 1: Psi is introduced much later so I couldn’t understand the bottom panel until I found its definition on page 4. Either the panel (or figure) should be moved or Psi explained earlier. Also, when Psi is explained a few sentences of further explanation or a couple of examples beyond the definition might help the reader to fully understand. After all, this parameter is directly tied to the eccentric breaks presented in this paper. (Unless my search function is not working properly, I see that the only time Fig 1 is only mentioned after Equation 5 on page 4, and this is after Figures 2 and 3 are mentioned.)

RESPONSE: The current figure 3, in which Psi is plotted, has been moved lower so that the definition of Psi is now introduced first. Additionally, under equation 5, I have further explained the relevance of Psi. 

7) Figure 2 – why put the legend in the middle panel left side? Middle panels - right side, retrograde disc. I am not sure I agree with how the peak of e moves as described in the text. It is certainly not easy to sort out how e changes from this figure. 

RESPONSE: In figure 1, the legend has been moved to the upper left panel. In section 2.2, paragraph 4, I have clarified the way that the eccentricity profile evolves and added some references to other work examining this behavior. Thank you for pointing out the confusing explanation in this section. 

8) Does the timescale of the expansion of the disc correspond to the viscous time scale?

RESPONSE: In the third paragraph of section 2.2 I have clarified that the disc expands on the viscous timescale. 

Section 2.1

9) given that no particles are injected during the simulation is your resolution still sufficient at larger radial distances to ensure that your results are interpreted correctly given you follow the disc over 75 orbital periods? 

RESPONSE: The retrograde circumprimary disc contains 200152 particles at 55 orbits (during the breaking event) and 161459 particles at the end of the simulation. Despite the dissipation of the disc, we have added a citation in paragraph 3 of the conclusions discussing the effects of resolution on the appearance of disc breaking features in SPH simulations. The retrograde circumprimary disc contains 200152 particles at 55 orbits (during the breaking event) and 161459 particles at the end of the simulation. 

10) is there a reference or explanation to why H/R is chosen as 0.01

RESPONSE: In paragraph 3 of section 2.1 I provide further justification for the chosen aspect ratio. 

11) Line 47 left side page 3, Section 2.2 “faster eccentricity growth” please give some approximate numbers

RESPONSE: Thank you for pointing out the description of eccentricity growth in the disc is unclear. This paragraph (paragraph 4 section 2.2) has been re-written to better communicate the disc behavior. The phrase "faster eccentricity growth" has been removed. 

12) can the authors approximate what you mean by slowly in the phrase “slowly
propagates inward” Perhaps it might be helpful to reference figure 3 upper panels or given the reader an idea of what you mean by an example, such as a comparison or the number of orbital periods over which this happens.

RESPONSE: This statement has been removed for clarity and the paragraph (paragraph 4 section 2.2) has been re-written. 

Section 2.3

13) The authors mention in the first paragraph, second sentence that in the retrograde disc, that the disc gets much closer to the companion. Could the authors provide a few estimates or comparison with the prograde case. Approximate values would be helpful.

RESPONSE: In the last sentence of the first paragraph we discuss the size of the disc in terms of the truncation radius, and provide the location in terms of semi-major axis. I have added a comparison to the prograde disc's truncation radius. Earlier in the paragraph I reiterate the location of the binary orbit. 

14) In the first paragraph of 2.3, details about the surface density with semi-major axis are explored in Figure 2 before the overall figure is introduced. It might be nice to have a few sentences to introduce the figure and state what is shown in the figure before diving into specifics.

RESPONSE: I have introduced all of the panels of figure 1 in the first paragraph of section 2.3. Now the figure is introduced in entirety before discussing the features of the plot. 

15) In this same first paragraph, truncation is mentioned as happening. However, nowhere do the authors explain how they determine truncation. Also, the fact that in the figure it looks like the outer disc continues to expand with time adds to the confusion.

RESPONSE: In the bottom of paragraph 1, section 2.3, we add a clarifying statement about the truncation radius. We also describe truncation in paragraph 3 of section 2.2. 

16) How long does it take for the retrograde to extend?

RESPONSE: In the first paragraph of section 2.3, I have clarified that the disc becomes truncated by 50 orbits, at which point it is no longer expanding, and in fact the outer edge then begins to shrink. 

17) At end of the first paragraph of this section– what causes the shrinking of the truncation?

RESPONSE: In beginning of the second paragraph, I specify that the shrinking of the truncation radius described in paragraph 1 is due to apsidal precession. In this paragraph I also add a more detailed description of the retrograde disc's arg. of periapsis evolution for figure 2. To accommodate this additional information, I add the description of the bottom right panel of Fig 1 to the next paragraph. 

18) Also, in this paragraph, the truncation is mentioned as significant at 50 orbital periods at a radius of a of 55 R. When I go back to Figure 1 or Figure 2, I don’t easily see this. I can see the Psi changes significantly in the bottom panels of Figure 1 , yet Psi has not yet been defined and explained yet. It would be nice if the authors could show the breaks on the 2D plots. Sorry for mentioning this again but it would be extremely helpful to show the breaks.

RESPONSE: We have restricted the axes of the top panels of the current figure 1 to show the surface density lines more clearly. The change in slope of the surface density line, signifying truncation, is now more visible in the t = 50 orbits line. 

19) Finally, in Figure 2, why are there bolded lines in the bottom panels. These line styles are not consistent with the upper panels. Note that there is only one legend, and these line styles are not in the legend. 

RESPONSE: We have changed the line styles in the bottom row of figure 1 (previously figure 2) to now match the rest of the figure.

20) Figure 3 is discussed in pieces similar to what was done for Figure 2. I would like to see the figures introduced in entirety in the text in the order that they appear.

RESPONSE: Figure 3 is now introduced in the second paragraph of section 2.3. Due to this change there are some small wording changes when referencing the panels of figure 3 later in this section. 

21) Psi is finally explained despite being plotted in the bottom of figure 1 - why does Psi vary so much in the bottom panels in figure 1 – is this real? How many particles are still in the calculation given it has been dissipating over 75 orbital periods. Is Psi an average of all the remaining particles at a given a?

RESPONSE: We have clarified that a large value of Psi represents a sudden jump in eccentricity. This is why it is a good measure (in conjunction with a dip in the surface density) of this kind of breaking. I have also slightly restricted the range of the horizontal axes of the Psi panels to better match figure 1 (see changes described in point 5). Despite the loss of particles throughout the simulation, in the third paragraph of section 4 we have given evidence that the break should only become stronger given a higher resolution. 

22) why is the equation solved for small e – aren’t we checking the retrograde case for larger e

RESPONSE: The linear evolutionary equation is only applicable for small eccentricity. Thus, to approximate the test particle behavior with the linear evolutionary equation, we must solve for small e. 

23) only the linear case for 30 R star is presented and I wondered why not present 50 as well as was done for the test particle?

RESPONSE: We have highlighted that at larger initial separation (i.e. at a = 50 solar radii) the linear theory can not fully describe the particle's behavior. This is why we do not choose to include it in figure 2.

25) It is probably worthwhile to remind the reader that you only consider coplanar discs

RESPONSE: In the first sentence of section 4 we have added the term "coplanar".

24) and 26) could the same phenomena happen for a tipped prograde disc since it could grow bigger? are the conclusions too strong if the prograde disc could grow larger if it were tipped?

RESPONSE: We have softened the language in the second paragraph of section 4 to acknowledge that this breaking mechanism may be able to operate for prograde discs with different parameters (such as tilting). We provide a recent example of eccentric breaking occurring in a prograde disc, but due to other eccentricity growth mechanisms besides forced eccentricity.

27) is there any way to connect if this phenomena of changes in eccentricity to the period in the X-ray variability

RESPONSE: We have added a prediction for the X-ray variability based on the potential for the eccentricity oscillations in the disc to continue. 

28) could the breaks affect the amount accretion from this scenario? I think it might be nice to comment how this interesting phenomenon might affect the bigger picture of accretion onto the companion and the variability of this accretion

RESPONSE: Although it is beyond the scope of this work to discuss how the breaking may influence the accretion onto the companion, we have emphasized that the break may impact the emission spectra where there is a contribution from the disc. 

